JOG3R: Towards 3D-Consistent Video Generators

Emergent capabilities of image generators have led to many impactful zero- or few-shot applications. Inspired by this success, we investigate whether video generators similarly exhibit 3D-awareness. Using structure-from-motion as a 3D-aware task, we test if intermediate features of a video generator - OpenSora in our case - can support camera pose estimation. Surprisingly, at first, we only find a weak correlation between the two tasks. Deeper investigation reveals that although the video generator produces plausible video frames, the frames themselves are not truly 3D-consistent. Instead, we propose to jointly train for the two tasks, using photometric generation and 3D aware errors. Specifically, we find that SoTA video generation and camera pose estimation (i.e.,DUSt3R [79]) networks share common structures, and propose an architecture that unifies the two. The proposed unified model, named \nameMethod, produces camera pose estimates with competitive quality while producing 3D-consistent videos. In summary, we propose the first unified video generator that is 3D-consistent, generates realistic video frames, and can potentially be repurposed for other 3D-aware tasks.

==> macro.tex <==
\usepackage{adjustbox}
\usepackage{bm}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{color, colortbl}
\usepackage{pifont}
\usepackage{xspace}
%
\usepackage[dvipsnames]{xcolor}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\iid{i.i.d\onedot} \def\wolog{w.l.o.g\onedot}
\def\etal{\emph{et al}\onedot}
\newcommand\minisection[1]{\vspace{1mm}\noindent \textbf{#1}}

% \newcommand{\red}[1]{{\color{red}#1}}
% \newcommand{\todo}[1]{{\color{red}#1}}
% \newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}



\newcommand{\nameCOLOR}[1]{\textcolor{black}{#1}}
\newcommand{\nameMethod}{\nameCOLOR{\mbox{JOG3R}}\xspace}
\newcommand{\faster}{\nameMethod}
\newcommand{\duster}{\nameCOLOR{\mbox{DUSt3R}}\xspace}
\newcommand{\meter}{\nameCOLOR{\mbox{MEt3R}}\xspace}
\newcommand{\opensora}{\nameCOLOR{\mbox{OpenSora}}\xspace}
\newcommand{\dit}{\nameCOLOR{\mbox{DiT}}\xspace}
\newcommand{\sfm}{\nameCOLOR{\mbox{SfM}}\xspace}
\newcommand{\realestate}{\nameCOLOR{\mbox{RealEstate10K}}\xspace}

\newcommand{\latent}{z\xspace}
\newcommand{\timestep}{t\xspace}
\newcommand{\noisylatent}{z_{\timestep}\xspace}
\newcommand{\prompt}{y\xspace}
\newcommand{\pointmap}{X\xspace}
\newcommand{\pointmaponeone}{X^{1,1}\xspace}
\newcommand{\pointmaptwoone}{X^{2,1}\xspace}
\newcommand{\pointmaponetwo}{X^{1,2}\xspace}
\newcommand{\pointmaptwotwo}{X^{2,2}\xspace}
\newcommand{\genloss}{\mathcal{L}_\text{gen}\xspace}
\newcommand{\recloss}{\mathcal{L}_\text{rec}\xspace}
\newcommand{\flcloss}{\mathcal{L}_\text{fl}\xspace}
\newcommand{\temploss}{\mathcal{L}_\text{tranl}\xspace}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

% \newcommand{\hmr}{\nameCOLOR{\mbox{HMR}}\xspace}



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/01_intro_old.tex <==
\section{Introduction}

Building on breakthroughs in foundational image models~\cite{rombach2021highresolution}, video diffusion models have advanced rapidly in recent years, resulting in numerous commercial and open-source models~\citep{guo2023animatediff,opensora,videoworldsimulators2024,menapace2024snap,blattmann2023stable}.
Trained on large-scale datasets like WebVid-10M \citep{Bain21} and Panda-70M \citep{panda70m}, these models generate realistic, diverse, and temporally smooth videos from text or image prompts.

%para3
% In addition to generating high-quality content, foundational generative models have recently been used as \emph{feature extractors} where intermediate features are used for tackling various analysis tasks (\eg, correspondence, semantic segmentation, etc.~\cite{tang2023emergent,dutt2024diffusion}). 
Beyond generating high-quality content, foundational generative models have recently been employed as \emph{feature extractors}, utilizing their intermediate features to tackle various analysis tasks such as correspondence matching and semantic segmentation \cite{tang2023emergent,dutt2024diffusion}.
% Specifically, even though trained on 2D data only, image generators have been shown to have emergent behavior to facilitate 3D-aware tasks~\cite{elbanani2024probing}. 
Notably, even though trained exclusively on 2D data, image generators have demonstrated emergent abilities for 3D-aware tasks~\cite{prob3d}.
Inspired by this success, we ask \textit{if the pre-trained video generators have similar emergent behavior towards 3D awareness.} 
To investigate this, we pick the classical structure-from-motion (SfM) as the target 3D task, as it requires reasoning about both scene geometry and the relative viewpoint changes across frames.

%para 2
In an exciting recent development, \duster~\citep{dust3r_cvpr24} demonstrated that the long-standing optimization-based structure-from-motion framework for camera estimation can be directly replaced by the forward pass of a dedicated network that has been trained to establish correspondence between any given pair of images. %This is in contrast to the current SoTA in optimization-based approach for structure-from-motion GLOMAP~\citep{pan2024global}.  
We observe that the ViT backbone in \duster actually shares many architectural designs in common with the Diffusion Transformers (DiT) backbone in state-of-the-art video generators.
This encourages us to investigate whether the intermediate features of a DiT-based video generation model, OpenSora in our setting, can be repurposed for the task of camera pose estimation.
% Hence, beyond real-world videos, we investigate whether the intermediate features of a video generation model, OpenSora in our setting, can be repurposed towards the 3D task of camera pose estimation. 

To facilitate our study, 
in this paper, we first present a novel architecture unifying video generation with camera pose estimation, which we refer to as \textit{JOint Generation and 3D camera Reconstruction}, in short \nameMethod. In particular, we attach \duster like prediction modules to a video generation network which are responsible for camera pose estimation.
Being a unified model, \nameMethod can generate videos (T2V), estimate camera poses given a video (V2C), or do both in one go (T2V+C).
We perform a thorough study on both tasks under the \nameMethod framework. We first explore if video generator features natively have 3D awareness by routing raw intermediate features from the pre-trained video generator to the camera pose estimation prediction heads. We then investigate whether the features can be further adapted towards camera pose estimation. In particular, we test whether with fine-tuning one can produce video generator features that can also be reused for improved camera tracking. Finally, we analyze the effect of such fine-tuning on generation quality. Our experiments show that while video generation features exhibit some 3D awareness natively (\ie, obtained from pre-trained generator directly), adapting them with additional supervision on the camera pose estimation task significantly boosts their 3D awareness. This additional supervision produces competitive camera pose estimations compared to state-of-the-art solutions without resulting in quality degradation in generated videos. 

%We present a \textit{JOint Generation and 3d camera Reconstruction} network, in short \nameMethod, that combines video generation with camera pose estimation into a single network, and can be supervised with generation and 3D reconstruction losses. We show that this does not cause a loss in video quality when setting a new SoTA with respect to camera tracking on real video using a feedforward network (see Figure~\ref{fig:output_modes}). We find that training with camera reconstruction leads to improved video generation, leading to an improved FVD score on the RealEstate10K-test. 

\if0
We propose a network for joint video generation w/ correspondence, thus encouraging the network to produce more 3d consistent results. We demonstrate that this leads to better reconstruction and we do not need multiple networks. Although the visual quality of the results are not better compared to vanilla video generators, ours (we need a name) is better in terms of 3d consistency

%para 4
a bit of details of how; residual networks, instead of directly using features, finetuned features work better, etc.

The goal of this paper is to study the 3D spatial awareness of video diffusion models. Specifically, how suitable are the features extracted from off-the-shelf video models for camera tracking?
Next, if finetuning is allowed, then a) how much better tracking can we deliver? b) can we maintain (or even improve) video generation quality?

\fi

%para 5
%summary of evaluation; why is this an important result

In summary, our contributions include:
\begin{itemize}
    \item Extensive experimentation and study on how well the video features can be used for 3D camera estimation and ablating the various design choices. 
    \item The first unified model that can both generate videos and estimate 3D cameras (see Figure~\ref{fig:teaser}). We refer to this model as \textit{JOint Generation and 3D camera Reconstruction} network, in short \nameMethod.
    % and 
    %\item Reporting SoTA video-based camera tracking results on both RealEstate10k-test and DL3DV10K datasets. 
\end{itemize}
% \begin{figure*}[t!]
% \begin{center}
% \includegraphics[width=\linewidth]{figures/teaser.pdf}
% \end{center}
% \vspace{-5mm}
% \caption{\nameMethod is a versatile model that (a)~generates a video from text, (b)~reconstructs 3D camera motion given a video, and (c)~simultaneously generates a video and corresponding camera motion.
% % \TODO{replace the image with overlaying video frames and put camera paths}
% The camera trajectories obtained in (b) and (c) are consistent.}
% \label{fig:output_modes}
% \end{figure*}

==> sec/03_setp.tex <==
\section{Problem Setup}
The goal of our experiments is to evaluate the 3D awareness of visual foundation models: i.e., large-scale pretrained models that are proposed as general backbones for a wide variety of downstream tasks or applications. Specifically, we hope to answer the following questions: 1. Do models learn to represent the visible surface? 2. Are the representations consistent across views? 3. Howdoes the training objective impact 3D awareness?

\minisection{Model.} We use \opensora

==> sec/04_experiments_old.tex <==
\section{Experiments}
We evaluate the design choices in two main aspects. 
We follow standard approaches to assess the generated video quality (T2V) while validating the accuracy of camera pose estimation on real videos (V2C). We further provide results for jointly generating videos along with camera pose estimation (T2V+C). Since there is no ground truth in this case, we focus on and report self-consistency.
\subsection{Setup}
\minisection{Data.} 
We choose \realestate \cite{zhou2018stereo} as the dataset, which has around 65K video clips paired with camera parameter annotations. 
We use the captions of \realestate provided in \cite{cameractrl} and also follow their train/test split.
As pre-processing, we pre-compute the VAE latents of the video frames and the T5 text embeddings of the captions. 
\textcolor{red}{
We sample $F$=16 frames from the original sequences with a frame stride randomly chosen from $\{1,2,4,8\}$ and 0.5 probability to reverse the frame order.
}
To obtain point map annotation $\bar{\pointmap}$, we estimate metric depth with ZoeDepth \citep{bhat2023zoedepth}, un-project it to 3D and transform to the coordinate of the first frame using the camera parameters in \realestate.
All camera extrinsic parameters are expressed w.r.t.~the first frame.

In addition, we consider DL3DV10K \citep{ling2024dl3dv}, which also provides camera annotations, as an additional test set. We choose a random set of 70 videos for testing and caption the first frame of each video using \cite{li-etal-2023-lavis}. We prepare point map annotations using ZoeDepth \citep{bhat2023zoedepth}. 
%, similar to the RealEstate10K dataset.

\begin{figure*}[h]
\begin{center}
\includegraphics[width=\linewidth]{figures/v2c_quali.pdf}
\end{center}
\vspace{-2mm}
\caption{\textbf{Qualitative camera pose estimation (V2C) results.} Red to purple indicates the progression from the first to the last frame. 
% The last row indicates a failure case. Please see suppmat.~for videos and more analysis.
}
\label{fig:rec-visuals}
\end{figure*}

\begin{figure*}[h]
\begin{center}
\includegraphics[width=\linewidth]{figures/t2vc_quali.pdf}
\end{center}
\vspace{-5mm}
\caption{\textbf{Qualitative generation T2V+C results.} It is coherent with the camera paths from T2V$\rightarrow$V2C. Please see suppmat.~for videos.}
\label{fig:t2vc_quali}
\end{figure*}


\begin{table*}
\begin{center}
\footnotesize
\begin{tabular}{lccrrrrr}
\toprule
 Backbone / Method & $\genloss$ & $\flcloss$ \& $\temploss$& Rot.~err.~($\degree$) $\downarrow$ &  Transl.~err.~($\degree$) $\downarrow$ & RRA@5$\degree$ $\uparrow$ &  RTA@5$\degree$  $\uparrow$  & mAA@30$\degree$ $\uparrow$ \\
\midrule  \midrule
% 0a.~frozen DiT & head & n.a. & \cmark & 99.18 & 59.33 & 0\% & 0.40\% & 0.1\%\\
1a.~frozen DiT  & n.a. & \cmark & 0.40 & 26.72 & 99.80\% & 11.63\% & 38.40\%  \\
% (1a) \nameMethod w/o $\genloss$& 0.36	& 33.09	& 99.71\%	& 12.18\%	& 34.55\%  \\
1b.~trainable DiT  & \xmark & \cmark & \textcolor{red}{0.28} & \textcolor{red}{21.13} & \textcolor{red}{99.90\%} & \textcolor{red}{19.23\%} & \textcolor{red}{49.49\%} \\
% ours w/o $\recloss$  &  &  &   \\
% \todo{\nameMethod (ours) }  & 0.36	& 32.73 & 99.65\% & 10.62\% &	35.03\%  \\
% \rowcolor{lightgray}
1c.~trainable DiT (\nameMethod) & \cmark & \cmark &  \textcolor{blue}{0.29}	& \textcolor{blue}{22.15} & \textcolor{blue}{99.79\%} & \textcolor{blue}{19.18\%} &	\textcolor{blue}{47.25\%}  \\
% 1c.~trainable DiT & w/o $\flcloss$ at test time  & \textcolor{red}{0.28}	&  29.82 & 99.78\% &  15.76\% &	 39.86\%  \\
1d.~trainable DiT    & \cmark & \xmark & 0.37	& 32.66 & 99.77\% & 13.16\% &	35.62\%  \\
\midrule
2a.~DUSt3R$^\dagger$ \cite{dust3r_cvpr24}  & n.a. & \xmark & 0.77 & 36.61 & 97.56\% & 7.54\%& 30.13\%\\
2b.~DUSt3R$^\dagger$ \cite{dust3r_cvpr24}  & n.a. & \cmark      & 0.53 & 27.86 & 99.12\% & 13.70\% & 40.20\%\\
2c.~DUSt3R* \cite{dust3r_cvpr24}  & n.a. & \cmark & \textcolor{red}{0.23} & \textcolor{red}{9.17} & \textcolor{red}{99.90\%} & \textcolor{red}{54.17\%} & \textcolor{red}{75.50\%} \\
2d.~DUSt3R$^0$ \cite{dust3r_cvpr24} & n.a. & \cmark & \textcolor{blue}{0.32} & \textcolor{blue}{20.66} & \textcolor{blue}{99.70\%} & \textcolor{blue}{15.33\%} & \textcolor{blue}{47.47\%}\\
\midrule
3.~GLOMAP \cite{pan2024glomap} & n.a. & n.a.   & 0.96 & 19.55 & 96.86\% & 25.92\% & 55.82\% \\
 \bottomrule
 \end{tabular}
\end{center}
\vspace{-2mm}
  \caption{
 \textbf{V2C error comparison on RealEstate10K-test.} DUSt3R\textsuperscript{$\dagger$} indicates pretrained \duster weights, whereas DUSt3R* is further trained with the same training set as our method -- RealEstate10K-train. DUSt3R$^0$ denotes training with RealEstate10K-train from scratch without initializing with pretrained weights. \textcolor{red}{Red}: best in the sub-table; \textcolor{blue}{blue}: second place in the sub-table.
 }
 \label{tab:rec_quanti}
 \vspace{-1mm}
\end{table*}

\begin{table*}
\begin{center}
\footnotesize
\begin{tabular}{lccrrrrr}
\toprule
 Backbone / Method & $\genloss$ & $\flcloss$ \& $\temploss$& Rot.~err.~($\degree$) $\downarrow$ & Transl.~err.~($\degree$) $\downarrow$ & RRA@5$\degree$ $\uparrow$ &  RTA@5$\degree$  $\uparrow$  & mAA@30$\degree$ $\uparrow$ \\
\midrule  \midrule
1a.~frozen DiT  & n.a. & \cmark & 6.49 & 39.53 & 65.06\% & 2.81\% & 19.70\%  \\
1b.~trainable DiT  & \xmark & \cmark & \textcolor{blue}{4.54} & \textcolor{blue}{30.05} & \textcolor{blue}{76.27}\% & \textcolor{red}{7.88\%} & \textcolor{blue}{33.60\%}\\
% \rowcolor{lightgray}
1c.~trainable DiT (\nameMethod) & \cmark & \cmark & \textcolor{red}{4.20}	& \textcolor{red}{29.17} &\textcolor{red}{78.63\%}& \textcolor{blue}{7.86\%} & \textcolor{red}{34.22\%} \\
1d.~trainable DiT    & \cmark & \xmark & 6.94	& 41.11 & 62.43\% & 2.66\% &	17.18\% \\
\midrule
2a.~DUSt3R$^\dagger$ \cite{dust3r_cvpr24}  & n.a. & \xmark & \textcolor{blue}{1.64} & 20.10 & \textcolor{blue}{96.25\%} & 37.03\%& 55.97\% \\
2b.~DUSt3R$^\dagger$ \cite{dust3r_cvpr24}  & n.a. & \cmark      & \textcolor{red}{1.33}& \textcolor{blue}{14.75} & \textcolor{red}{97.53\%} & \textcolor{red}{47.03\%} & \textcolor{red}{65.73\%}\\
2c.~DUSt3R* \cite{dust3r_cvpr24}  & n.a. & \cmark & 1.83 & \textcolor{red}{14.17} & 93.63\% & \textcolor{blue}{38.57\%} & \textcolor{blue}{64.40\%}\\
2d.~DUSt3R$^0$ \cite{dust3r_cvpr24} & n.a. & \cmark & 6.25 & 39.37 & 65.84\% & 3.41\% & 19.73\%\\
\midrule
3.~GLOMAP \cite{pan2024glomap} & n.a. & n.a.   & 0.53	& 4.92 & 98.03\%& 87.39\% & 90.39\% \\
 \bottomrule
 \end{tabular}
\end{center}
\vspace{-2mm}
  \caption{
 \textbf{V2C error comparison on DL3DV10K.} \textcolor{red}{Red}: best in the sub-table; \textcolor{blue}{blue}: second place in the sub-table. }
 \label{tab:rec_quanti_dl3dv}
  \vspace{-2mm}
\end{table*}

\minisection{Baselines.}
Since there is no existing method that can perform both video generation and camera pose estimation jointly, we can only compare to task-specific methods. 
We use the original pair-wise method \duster \cite{dust3r_cvpr24} with linear head and a global SfM method GLOMAP \citep{pan2024glomap} as camera pose estimation methods to provide a reference for our analysis.
For \duster we consider three variants: (i)~off-the-shelf pretrained weights (DUSt3R\textsuperscript{$\dagger$}), (ii)~initialized with pretrained weights and trained with the same data as ours (DUSt3R*), and (iii)~trained from scratch with the same data as ours (DUSt3R$^0$). 
In all three variants, we perform the final global optimization step with our newly introduced temporal loss $\temploss$ and $\flcloss$. 
For video generation we consider the pretrained OpenSora as a baseline. 
% For GLOMAP we report the results before the global bundle adjustment part. 

\minisection{Metrics.}
We validate the quality of camera tracking on real videos (V2C) by comparing the estimated camera poses $(\textbf{R},\textbf{t})$ with the ground truth poses $(\bar{\textbf{R}},\bar{\textbf{t}})$. 
For rotation, we compute the relative error between two rotation matrices \cite{wang2023posediffusion}. 
Since the estimated and ground-truth translation can differ in scale, we follow \cite{wang2023posediffusion} to compute the angle between the two normalized translation vectors, \ie, $\arccos(\textbf{t}^\top\bar{\textbf{t}}/(\|\textbf{t}\|\|\bar{\textbf{t}}\|))$.
Besides reporting the average of the two errors, we also follow \cite{dust3r_cvpr24} to report Relative Rotation Accuracy (RRA) and Relative Translation Accuracy (RTA), \ie, the percentage of camera pairs with rotation/translation error below a threshold.
Due to the small number of frames handled by the video generator, each videos sequence exhibits small rotation variation. Hence, we select a threshold 5$\degree$ to report RTA@5 and RRA@5. 
Additionally, we calculate the mean Average Accuracy (mAA@30), defined as the area under the curve accuracy of the angular differences at min(RRA@30, RTA@30).
We also use FID~\citep{fid} and FVD~\citep{unterthiner2019fvd} to measure image and video quality, respectively. %, ensuring that our method maintains high generation quality.

\subsection{Reconstruction Evaluation}
In Table~\ref{tab:rec_quanti}, we compare the camera pose estimation (V2C) errors on RealEstate10K-test and report the errors of withheld DL3DV10K in Table~\ref{tab:rec_quanti_dl3dv}.
In both tables, even when there are decoders trained to perform reconstruction from the Sora features, freezing Sora backbone still leads to noticeably worse results than the trainable counterparts (row 1a vs.~1b or 1c).
This means \textit{raw features from pretrained video generators are insufficient for camera pose estimation}.  
Comparing rows 1b and 1c of two tables, we see that models trained without generation loss $\genloss$ lead to overall similar results to our full model, suggesting that \textit{retaining generation ability has limited effect on reconstruction}.

% \textcolor{red}{
Our full method, \nameMethod, performs overall better than pretrained DUSt3R$^\dagger$ on \realestate, cf.,~Table \ref{tab:rec_quanti} row 1c and 2b.
When trained with the same RealEstate10K-train, \nameMethod still has on-par reconstruction quality compared with the from-scratch trained DUSt3R$^0$, but not DUSt3R*.
This suggests pretrained DUSt3R weights contain richer information for camera pose estimation than the pretrained OpenSora weights.
% When we replace the original \duster decoders with full 3D attention blocks (0), we obtain on-par results with a marginal drop in accuracy.
Meanwhile, the overall results in Table \ref{tab:rec_quanti_dl3dv} suggests \nameMethod is not as competitive in generalization, which we attribute to the faster motion in DL3DV10K.  
Since DUSt3R$^\dagger$ and DUSt3R* contain pretrained knowledge learned from matching wide-baseline view pairs, they naturally perform better than DUSt3R$^0$ in DL3DV10K, which is solely trained with RealEstate10K-train.
% }
We also report the results of GLOMAP~\citep{pan2024glomap}, an optimization based state-of-the-art SFM method.
In row 3 of both tables, we observe it does surpass most methods, except for DUSt3R* in Table \ref{tab:rec_quanti}.  
% The margin is even larger when the overlap between consecutive frames gets smaller, like in DL3DV10K. 
This demonstrate the strength of the optimization-based global method. 
% In Table \ref{tab:rec_quanti} row 3, we observe it does surpass most methods (except for DUSt3R*) in RealEstate10K, where videos often contain smaller motion and hence smaller baselines for each stereo pair.  
% When the overlap between consecutive frames gets smaller, like in DL3DV10K, such a video-based method struggles and our method actually yields lower errors than GLOMAP. 
% \TODO{State our observation once we have the final results.}

Figure~\ref{fig:rec-visuals} shows the qualitative comparison of our method and baselines (with $\flcloss$ \& $\temploss$).
Since camera poses are estimated through registration, which builds 3D correspondences along the way, we visualize the final camera trajectories as well as the correspondence between the first and the last frame.
One can see that our method produces good camera trajectories similar to pretrained \duster, which is a method tailored for reconstruction only, but no generation. In some cases ours are closer to ground truth camera paths.
% In the last row we show a failure case where \textit{both} our method and \duster fail to estimate reasonable camera poses. 
% We hypothesize this is due to the infinite depth in the sky region which could cause inconsistent scale normalization across each stereo pair.

%\TODO{State our observation once we have the final results.}

\subsection{Generation Evaluation}
For each method, we generate 180 videos using the captions in RealEstate10K-test  and report the FID/FVD against  the real images/videos in RealEstate10K-test. 
Table~\ref{tab:gen_quanti} suggests that our full model generates more realistic images/videos than pretrained OpenSora (row 1c vs.~2).
When ablating the generation loss $\genloss$, the quality slightly degrades compared to our full model (row 1c vs.~1a).
This is intuitive because without the generation loss, there is nothing to enforce the model to retain its full generation capability. See also supplemental videos. 
It is worth noting that row 1b corresponds to a baseline where $\recloss$ is disabled by removing \duster decoders/heads, \ie, it is equivalent to standard diffusion model finetuning except only the weights of the temporal attention layers are updated. 
We see that removing $\recloss$ leads to different impacts on FID and FVD.
Therefore, we conclude \textit{camera pose estimation has mixed impact on video generation}.
Figure~\ref{fig:t2v_quali} shows a few examples of videos generated by \nameMethod.
% Since our method aims to generate videos, we argue FVD is a more important metric to measure the quality. 
% As a result, the lower FVD of our full methdod (1c) suggests \textit{learning camera pose estimation positively impacts the quality of video generation}.   
% and the qualitative comparison also confirms the benefit of reconstruction loss $\recloss$.
\if False
\begin{table}
\begin{center}
\footnotesize
\begin{tabular}{lrr}
\toprule
 Method &  FID $\downarrow$ & FVD $\downarrow$  \\
\midrule  \midrule
% 1a.~ours w/o $\genloss$  & 110.40 & 1898.72    \\
1a.~ours w/o $\genloss$  &  &     \\
1b.~ours w/o $\recloss$  & 88.02 & 1440.92  \\
1c.~\nameMethod (ours)   & 94.75	&  \\
\midrule
2.~pretrained OpenSora & 115.36 & 1872.41 \\
 \bottomrule
 \end{tabular}
\end{center}
  \caption{
 \textbf{Generation quality comparison.} We compute the FID and FVD with RealEstate10K-test. }
 \label{tab:gen_quanti}
\end{table} 
\fi

\begin{table}
\begin{center}
\footnotesize
\begin{tabular}{lccrr}
\toprule
Backbone / Method & $\genloss$ & $\recloss$& FID $\downarrow$ & FVD $\downarrow$  \\
\midrule  \midrule
1a.~trainable DiT  & \xmark & \cmark & 94.52 & 1797.07    \\
1b.~finetuned OpenSora  & \cmark & \xmark & 88.02 & \textbf{1440.92}  \\
1c.~trainable DiT (\nameMethod)  & \cmark & \cmark & \textbf{79.94}	&  1742.73  \\
\midrule
2.~pretrained OpenSora & n.a. & n.a. & 115.36 & 1872.41 \\
 \bottomrule
 \end{tabular}
\end{center}
\vspace{-2mm}
  \caption{
 \textbf{Generation quality comparison.} We compute the FID and FVD with the RealEstate10K-test. }
 \label{tab:gen_quanti}
 \vspace{-2mm}
\end{table} 


\subsection{Discussion}
\minisection{Self consistency of T2V$\rightarrow$V2C and T2V+C}.
Since \nameMethod can \textit{generate} camera trajectories in two ways: cascading T2V and V2C or the tightly coupled T2V+C pipeline, it is worth comparing how much the two results differ.
We run the two pipelines with 100 prompts and report 0.45$\degree$ average difference in rotation and 19.20$\degree$ in translation; both are low errors compared with the corresponding numbers in Table \ref{tab:rec_quanti} and \ref{tab:rec_quanti_dl3dv}, indicating that the camera poses from joint T2V+C pipeline is consistent with T2V$\rightarrow$V2C.
The qualitative results in Figure~\ref{fig:t2vc_quali} also confirm this conclusion.
% Naturally one We compare the consistency 
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{figures/t2v_quali.pdf}
\end{center}
\vspace{-2mm}
\caption{\textbf{Qualitative T2V generations.} Please see suppl.~videos.}
\label{fig:t2v_quali}
%\vspace{-2mm}
\end{figure}

\minisection{Synergy of two tasks.}
Our unified architecture enables multi-task training: generation loss $\genloss$ and reconstruction loss $\recloss$.
However, according to Table \ref{tab:rec_quanti} and \ref{tab:rec_quanti_dl3dv}, $\genloss$ does not have a significant positive impact on camera pose estimation, while in Table \ref{tab:gen_quanti}, $\recloss$ also has mixed impact on generation. Thus, we conclude that we \textit{do not observe a synergistic effect between two tasks}, at least in the framework of OpenSora 1.0.

% In both Table \ref{tab:rec_quanti} and \ref{tab:rec_quanti_dl3dv}, (1a) and (1b), we show that keeping the generation loss $\genloss$ helps the reconstruction branch attain better camera poses estimation.
% On the other hand, Table \ref{tab:gen_quanti} (1b) and (1c) also suggest that introducing the reconstruction task results in better video generation quality.
% Empirically, we demonstrate a synergy between two tasks -- learning to generate helps reconstruction; learning to reconstruct also helps generation. 
% It shares the same spirit with the known ``analysis and synthesis'' analogy, but our architectural design tightly couples them in one network and allows end-to-end training.

\minisection{Role of $\genloss$.}
Despite two tasks have no observable synergistic effect, we choose to enable $\genloss$ in our full method because it leads to on-par camera pose estimation results (Table \ref{tab:rec_quanti} and \ref{tab:rec_quanti_dl3dv}) and improved generation quality (Table \ref{tab:gen_quanti}).

\minisection{Value of \nameMethod.}
To our knowledge, \nameMethod is the first method that performs video generation and camera pose estimation jointly.
The new unified architecture enables end-to-end training of two tasks, and it opens up new research directions.
Without precedents, we can only compare with state-of-the-art methods in each task, which are dedicated specifically to solve the corresponding tasks.
Nonetheless, we still achieve on-par quantitative results in RealEstate10k (Table \ref{tab:rec_quanti}), and all qualitative figures confirm that \nameMethod generates realistic videos (T2V), estimates reasonably good camera paths (V2C) and they are self coherent (T2V+C).
% Despite not beating SoTA methods , we show in that 
% Even though two tasks have no observable synergistic effect, we choose to enable $\genloss$ in our full method because it leads to on-par camera pose estimation results (Table \ref{tab:rec_quanti} and \ref{tab:rec_quanti_dl3dv}) and improved generation quality.
